Large-Scale Public Data Improves Differentially Private Image Generation Quality

Public data has been frequently used to improve the privacy-accuracy trade-off of differentially private machine learning, but prior work largely assumes that this data come from the same distribution as the private. In this work, we look at how to use generic large-scale public data to improve the quality of differentially private image generation in Generative Adversarial Networks (GANs), and provide an improved method that uses public data effectively. Our method works under the assumption that the support of the public data distribution contains the support of the private; an example of this is when the public data come from a general-purpose internet-scale image source, while the private data consist of images of a specific type. Detailed evaluations show that our method achieves SOTA in terms of FID score and other metrics compared with existing methods that use public data, and can generate high-quality, photo-realistic images in a differentially private manner.

==> sections/experiment.tex <==
\section{EXPERIMENT}
\begin{table*}[t]
    \centering
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
    \toprule
        \multirow{2}{*}{\textbf{Method}} &  \multicolumn{5}{c|}{Cifar10} &  \multicolumn{5}{c}{ Pet}  \\
         \cmidrule{2-11}
         & $\varepsilon=10^6$    & $\varepsilon=10$  & $\varepsilon=3$   & $\varepsilon=1$  & $\varepsilon=0.1$   & $\varepsilon=10^6$    & $\varepsilon=10$  & $\varepsilon=3$   & $\varepsilon=1$  & $\varepsilon=0.1$   
         
          \\
        \midrule
        % Train images  &  \multicolumn{5}{c|}{3.3}	&  \multicolumn{5}{c}{10.8}     \\
        {\small Non-private IC-GAN}  &   \multicolumn{5}{c|}{16.3}	&   \multicolumn{5}{c}{29.8}  \\
        \midrule
        DP-GAN-FT  & 43.4	&55.8	&55.9	&56.0	&53.5  & 42.7	&131.1	&131.1	&131.1	&130.5\\
        DP-MEPF  & 36.9	&37.0	&41.8	&68.3	&296.5  &87.9	&74.8	&104.2	&109.3	&194.5\\
        DP-GAN-MI  &  \textbf{16.5} &	39.6&	51.7&	67.3&	114.9 & 38.0	&112.8	&168.4	&182.1	&173.3\\
        \midrule
        DP-MGE  & 34.0	& 34.0	& 34.0	& 34.0 & 35.5  &  76.6 & 76.4 & 77.1 & \textbf{78.9} & 161.2  \\
        DP-DRE  & 20.8	&\textbf{21.7}	&\textbf{21.6}	&\textbf{21.7}	&\textbf{28.8}  & \textbf{35.4} & \textbf{36.6} & \textbf{41.5} & 88.6 & \textbf{94.1} \\
        \midrule
        \midrule
        \multirow{2}{*}{\textbf{Method}} &  \multicolumn{5}{c|}{Car} & \multicolumn{5}{c}{Bird}\\
         \cmidrule{2-11}
         & $\varepsilon=10^6$    & $\varepsilon=10$  & $\varepsilon=3$   & $\varepsilon=1$  & $\varepsilon=0.1$   & $\varepsilon=10^6$    & $\varepsilon=10$  & $\varepsilon=3$   & $\varepsilon=1$  & $\varepsilon=0.1$   
         
          \\
        \midrule
        % Train images  &  \multicolumn{5}{c|}{2.8} &   \multicolumn{5}{c}{5.2}\\
        {\small Non-private IC-GAN}  &   \multicolumn{5}{c|}{13.8} &  \multicolumn{5}{c}{18.0} \\
        \midrule
        DP-GAN-FT  &  14.3	&158.8	&158.9	&158.8	&158.8 &   26.9	&140.0	&139.9	&139.8	&140.0\\
        DP-MEPF  &  80.7		&64.9	&105.3	&91.3	&132.2  &  55.3	&	66.4	&61.4	&64.9	&\textbf{103.8}\\
        DP-GAN-MI  &  \textbf{13.0}	&30.9	&203.6	&225.1	&236.7  &  \textbf{17.1}	&164.9	&183.8	&188.4	&189.0\\
        \midrule
        DP-MGE  &  17.8 & 17.7 & 17.7 & 17.7 & \textbf{65.4} & 27.0 & 26.8 & \textbf{26.8} & \textbf{26.9} & 105.4 \\
        DP-DRE  & 15.1 & \textbf{16.2} & \textbf{16.5} & \textbf{17.0} & 141.8 &  19.3 & \textbf{24.7} & 27.3 & 60.3 & 107.2\\
        \midrule
        \midrule
        \multirow{2}{*}{\textbf{Method}} &  \multicolumn{5}{c|}{ Objects-Grass}  & \multicolumn{5}{c}{Objects-Autumn}\\
         \cmidrule{2-11}
         & $\varepsilon=10^6$    & $\varepsilon=10$  & $\varepsilon=3$   & $\varepsilon=1$  & $\varepsilon=0.1$   & $\varepsilon=10^6$    & $\varepsilon=10$  & $\varepsilon=3$   & $\varepsilon=1$  & $\varepsilon=0.1$   
         
          \\
        \midrule
        % Train images  &  \multicolumn{5}{c|}{8.7}   &  \multicolumn{5}{c}{19.6} \\
        {\small Non-private IC-GAN}  &   \multicolumn{5}{c|}{19.9} & \multicolumn{5}{c}{37.3}  \\
        \midrule
        DP-GAN-FT  & 35.6	&81.0	&80.6	&81.4	&81.4  &  49.4	&92.2	&92.1	&92.3	&92.3\\
        DP-MEPF  &  91.9	&	80.3&	79.5&	86.6&	110.3  & 89.4	&93.2	&90.5	&104.7	&161.8\\
        DP-GAN-MI  &  \textbf{22.2}	& 82.2	&112.2	&129.7	&125.8  & \textbf{41.5}	&131.5	&139.8	&139.0	&144.6\\
        \midrule
        DP-MGE  & 58.7 & 58.8 & 58.9 & 59.2 & 67.0  & 75.2 & 75.2 & 75.4 & 76.3 & 102.5\\
        DP-DRE  & 26.9 & \textbf{27.5} & \textbf{28.2} & \textbf{27.8} & \textbf{46.6}  & 45.5 & \textbf{47.7} & \textbf{49.5} & \textbf{49.7} & \textbf{61.9}\\
        \bottomrule
    \end{tabular}
    \caption{FID score (lower is better) of generated data for 6 different private datasets.}
    \label{tab:fid_score}
\end{table*}

We now evaluate our methods and demonstrate their practical applicability in realistic image generation. In particular, this section aims to answer the following questions: 1. How do our proposed methods compare with existing baseline methods in terms of standard image-generation metrics? 2. How does DP-MGE compare with DP-DRE? 3.How do different methods in the literature compare in terms of image quality?

\subsection{Experiment set-up}
%\begin{table*}[]
%    \centering
%    \begin{tabular}{c|cccccc}
%    \toprule
%    \textbf{Dataset} & Cifar10 & Pet & Bird & Car & Objects-Grass & Objects-Autumn\\
%    \midrule
%    Size of Train. Set & \\
%    Resolution & 32 & 128 & 128 & 128 & 128 & 128\\
%    \bottomrule
%    \end{tabular}
%    \caption{Dataset statistics.}
%    \label{tab:data_stat}
%\end{table*}

\mypara{Datasets.} For all our experiments, we use ImageNet \citep{deng2009imagenet} as the public data, with the pretrained feature extractor $h$ and IC-GAN $g$ from \citet{casanova2021instance}\footnote{The pretrained models are from \url{https://github.com/facebookresearch/ic_gan}}.
%\kc{Move this to experimental details: The dimensionality of the feature space is $2048$.}

We use multiple private datasets -- CIFAR10~\citep{krizhevsky2009learning} (Cifar10), Oxford-IIIT Pet Dataset~\citep{parkhi2012cats} (Pet), Stanford Cars Dataset~\citep{KrauseStarkDengFei-Fei_3DRR2013} (Car), Caltech-UCSD Birds Dataset~\citep{wah2011caltech} (Bird), Nico+~\citep{zhang2022nico++} with Grass (Objects-grass) and Nico+ with Autumn (Objects-autumn). These are considerably smaller than Imagenet, and have sizes $50000$, $3680$, $5992$, $8144$, $16256$ and $7272$ respectively. Images in Cifar10 have resolution $32$ and we resize images from the other datasets to resolution $128$. We use the train split of each dataset for training the image generation algorithms and validation or test splits for evaluation.

\mypara{Algorithm set-up.} We evaluate both DP-MGE and DP-DRE. For DP-MGE, the normalization operator in the feature extractor $h$ ensures that the norm of the features $\|\bv_i\| \leq 1$, thus ensuring privacy (see Claim~\ref{clm:mge_dp}). For DP-DRE, we choose a two-layer MLP as our discriminator $D^{\dagger}_{\theta}$. More training details are provided in the Appendix. 

%\kc{put these details in the appendix} The hidden sizes are selected from $\{1, 4, 16, 64, 256\}$. The size of the validation set $V$ used in DP-DRE is $50000$, $50$ images per class in the ImageNet. The training details are in the appendix.


\mypara{Baselines.} We compare our methods with the following three baselines that all utilize public data; details on how they are trained are provided in the appendix. In all cases, for fair comparison, we try to keep the architectures as close to the IC-GAN architecture as possible.

% In addition to the private baselines below, we also report two non-private baselines: the scores for the training images, and the scores for images generated from the IC-GAN when the private data is directly input to it. The first serves as an upper bound for any image generation algorithm and the second is an upper bound for any IC-GAN based image generation algorithm.
In addition to the private baselines below, we also report a non-private baseline: the scores for images generated from the IC-GAN when the private data is directly input to it. This is an upper bound for any IC-GAN based image generation algorithm.

\textit{DP finetuning on private data (DP-GAN-FT)} finetunes a pretrained public GAN on private data with differential privacy. For our experiment, we train a GAN on Imagenet in the feature space described by the pretrained feature extractor $h$. Both the generator and discriminator of this GAN are $4$-layer MLPs. We sequentially combine the generator of this trained GAN with the IC-GAN generator, and its discriminator with the IC-GAN discriminator to get a complete unconditional GAN on Imagenet. The combined generator and discriminator are then finetuned together on the private data using a differentially private version of Adam. 


\textit{DP mean embedding with perceptual features (DP-MEPF)~\citep{harder2022differentially}} uses the public data to extract pretrained features, and calculates the first and second moments of the private data in the feature space with differential privacy. A generative model is then trained to generate data that matches these moments. For cifar10, we follow the same set-up\footnote{We use the code at \url{https://anonymous.4open.science/r/dp-mepf/README.md}} as in \citet{harder2022differentially} -- the pre-trained features are the perceptual features from each layer of the VGG-19 network~\citep{simonyan2014very} and the generator is a ResNet. For the other datasets, we pretrain a ResNet50 on ImageNet. We use BigGAN as the architecture of the generator and set the deep features as the output of the layer right before the last pooling layer.     	
    	 
\textit{DP-GAN with model inversion (DP-GAN-MI)~\citep{chen2021differentially}} pretrains an unconditional GAN on the public data and then trains a differentially private GAN in its latent space. To generate a new image, it first generates a latent vector via the private GAN, and passes it to the pretrained GAN. We use this procedure with the IC-GAN architecture, and train a differentially private GAN in the latent space of the feature extractor $h$. The private generator and discriminator both are $4$-layer MLPs.

 
%   	In our experiment, we train a GAN to generate the distribution of ImageNet in the latent space defined by the pretrained feature extractor $h$. 
%    	The generator $g^{\rm latent}$ in this GAN has the architecture of $4$-layer MLP with the hidden width $1024$ and latent dimensionality $128$.
%    	The discriminator $D^{\rm latent}$ is also a $4$-layer MLP with the hidden width $1024$.
%    	Then we squentialy combine the generator $g^{\rm latent}$ and the pretrained IC-GAN $g$ as the generator of an unconditional GAN on ImageNet.
%    	We also combine the pretrained feature extractor $h$ and the discriminator $D^{\rm latent}$ as the corresponding discriminator.
%	\kc{I did not understand this experimental setup. To be discussed.} \kc{Also: it sounds very complicated and needs some motivation.}	
    	
    
%\textit{DP mean embedding with perceptual features (DP-MEPF)~\cite{harder2022differentially}} uses the public data to extract pretrained features, and calculates the means and squared means of the private data in the feature space with differential privacy. A generative model is then trained to generate data that minimizes the distance between the means of features and the squared features among the generated images and the calculated means from the private data. For cifar10, we follow the same set-up\footnote{We use the code at \url{https://anonymous.4open.science/r/dp-mepf/README.md}} as in \cite{harder2022differentially} -- we set the pre-trained features as the perceptual features from each layer of the VGG-19 network \cite{simonyan2014very} and use a ResNet generator. For the other datasets, we pretrain a ResNet50 on ImageNet. We use BigGAN as the architecture of the generator and set the deep features as the output of the layer right before the last pooling layer. \kc{Are these the pre-trained features?} \kc{Is this too many details?}
    	
    	 
%\textit{DP-GAN with model inversion (DP-GAN-MI)~\cite{chen2021differentially}} pretrains an unconditional GAN on the public data and then trains a differentially private GAN in its latent space. To generate a new image, it first generates a latent vector via the private GAN, and passes it to the pretrained GAN. We use this procedure with the IC-GAN architecture, and train a differentially private GAN in the latent space of the feature extractor $h$. The private generator and discriminator both are $4$-layer MLPs.
%with latent dimension $25$ and hidden width selected from $\{32, 128\}$. \kc{does this look correct?}

\begin{table*}[t]
    \centering
    \begin{tabular}{c|cc|cc|cc|cc|cc}
    \toprule
%    \multirow{3}{*}{\textbf{Method}} & \multicolumn{10}{c}{Cifar10}\\
%    \cmidrule{2-11}
    \multirow{2}{*}{\textbf{Method}}& \multicolumn{2}{c|}{$\varepsilon=10^6$}& \multicolumn{2}{c|}{$\varepsilon=10$}& \multicolumn{2}{c|}{$\varepsilon=3$}& \multicolumn{2}{c|}{$\varepsilon=1$}& \multicolumn{2}{c}{$\varepsilon=0.1$}\\
%    \cmidrule{2-11}
    & Prec. & Rec.  & Prec. & Rec.  & Prec. & Rec.  & Prec. & Rec.  & Prec. & Rec. \\
    \midrule
    Non-private IC-GAN & \multicolumn{10}{c}{Precision: 0.950, Recall: 0.965}\\
    \midrule
        DP-GAN-FT  & 0.789 & 0.829 & 0.787 & 0.756 & 0.752 & 0.751 & 0.770 & 0.766 & 0.794 & 0.772\\
        DP-MEPF  &  0.910 & 0.873 & 0.913 & 0.880 & 0.903 & 0.835 & 0.820 & 0.658 & 0.013 & 0.000\\
        DP-GAN-MI  &  \textbf{0.957} & \textbf{0.944} & 0.825 & 0.741 & 0.865 & 0.670 & 0.749 & 0.544 & 0.392 & 0.527\\
        \midrule
        DP-MGE  & 0.910 & 0.786 & 0.916 & 0.781 & 0.910 & 0.778 & 0.905 & 0.798 & \textbf{0.917} & 0.790\\
        DP-DRE  & 0.952 & 0.920 & \textbf{0.961} & \textbf{0.929} & \textbf{0.930} & \textbf{0.931} & \textbf{0.928} & \textbf{0.937} & 0.880 & \textbf{0.901}\\
%    \midrule
%    \midrule
%    \multirow{3}{*}{\textbf{Method}} & \multicolumn{10}{c}{Pet}\\
%    \cmidrule{2-11}
%    \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{$\varepsilon=10^6$}& \multicolumn{2}{c|}{$\varepsilon=10$}& \multicolumn{2}{c|}{$\varepsilon=3$}& \multicolumn{2}{c|}{$\varepsilon=1$}& \multicolumn{2}{c}{$\varepsilon=0.1$}\\
%%    \cmidrule{2-11}
%    & Prec. & Rec.  & Prec. & Rec.  & Prec. & Rec.  & Prec. & Rec.  & Prec. & Rec. \\
%    \midrule
%        DP-GAN-FT  & 0.805 & 0.886 & 0.310 & 0.155 & 0.319 & 0.180 & 0.306 & 0.161 & 0.326 & 0.178\\
%        DP-MEPF  &  0.474 & 0.451 & 0.608 & 0.540 & 0.236 & 0.248 & 0.454 & 0.315 & 0.015 & 0.004\\
%        DP-GAN-MI  &  0.809 & 0.912 & 0.361 & 0.179 & 0.182 & 0.149 & 0.104 & 0.165 & 0.102 & 0.104\\
%        \midrule
%        DP-MGE  & 0.543 & 0.492 & 0.570 & 0.513 & 0.534 & 0.520 & \textbf{0.550} & 0.500 & 0.141 & 0.163\\
%        DP-DRE  & \textbf{0.822} & \textbf{0.920} & \textbf{0.812} & \textbf{0.900} & \textbf{0.848} & \textbf{0.846} & 0.542 & \textbf{0.643} & \textbf{0.585} & \textbf{0.518}\\
    \bottomrule
    \end{tabular}
    \caption{Precision and recall (higher is better) of our methods and baselines on Cifar10 dataset. See the Appendix for results of other five datasets.}
    \label{tab:prec_rec}
\end{table*}

\begin{figure}[t]
\centering
	\includegraphics[width=\linewidth]{sections/figs/result_figures/ndb_cifar10.pdf}
%	\includegraphics[width=\linewidth]{sections/figs/result_figures/ndb_OxfordIIITPet.pdf}
	\caption{The percentage of different bins NDB/K (lower is better) of our methods and baselines on Cifar10 dataset. Results of other five datasets are in the Appendix.}
	\label{fig:ndb}
\end{figure}

\begin{figure*}[t]
\centering
	\includegraphics[width=\linewidth]{sections/figs/examples.pdf}
	\caption{Examples of all algorithms ($\varepsilon=10$) across six datasets. More examples for different $\varepsilon$ are in the Appendix.}%Put this text back when we have more space: We see that DP-DRE and DP-MGE generate the most in-distribution images with high quality for all datasets except Object-Autumn. Other methods either generate many irrelevant out-of-distribution images (DP-GAN-FT, DP-GAN-MI) or have many artifacts (DP-MEPF). 
	\label{fig:examples}
\end{figure*}


\mypara{Evaluation Metrics.} Since there is no one perfect metric for evaluating generation quality, we use three popular metrics to measure the effectiveness of our methods. 

%For evaluating the generated images, we use the following metrics that measure the quality of the generated distribution compared with the private data distribution. 

The \textit{Frechet Inception Distance} (FID) Score \citep{heusel2017gans} measures the distance between the generated distribution and the target distribution by comparing the means and variances in a feature space computed from a pretrained Inception V3 model.  %Note that a smaller FID means better generation. 

The \textit{Precision and Recall}~\citep{sajjadi2018assessing} metric evaluates the distance between the target and the generated distributions along two separate dimensions -- precision, which measures the sample quality of the generation algorithm, and recall, which measures the proportion of the target distribution that is covered by the generated distribution. These two are evaluated in a feature space after clustering; as suggested by~\citet{sajjadi2018assessing}, we choose $K=20$ clusters and report the maximum of $F_8$ and $F_{1/8}$ for precision and recall.

\textit{Number of Different Bins (NDB)} \citep{richardson2018gans} compares the histogram of two distributions in the pixel space after clustering samples from the target distribution into bins. We choose $K=50$ clusters. %Smaller NDB is better.
 
%We rather than the deep feature space that is explored in the last two evaluations. 
%    First samples from the target distribution are clustered in the pixel space.
%    For each cluster $k$, we calculate the proportion $p_k$ of target samples that are assigned to this cluster and also the proportion $p_k'$ of generated samples.
%    If target distribution and generated distribution are the same, $p_k$ and $p_k'$ would be very close.
%    NDB measures the number of clusters that $p_k$ and $p_k'$ are significantly different.
%    We choose the cluster number as $K=50$.
\subsection{Results}

We run methods on each dataset with $\varepsilon\in\{10^6, 10, 3, 1, 0.1\}$ and $\delta=10^{-5}$. 
Table~\ref{tab:fid_score} reports the FID scores of all algorithms on all the private datasets.
Table~\ref{tab:prec_rec} and Figure~\ref{fig:ndb} present the precision and recall and NDB on Cifar10; the results for the other five datasets are presented in the Appendix. 
We find that the conclusions drawn from the precision and recall and NDB tables largely agree with the results of the FID scores. 

%Our next discussions are based on the results of FID scores (Table~\ref{tab:fid_score}).
%The results of precision and recall (Table~\ref{tab:prec_rec}) and NDB (Figure~\ref{fig:ndb}) constantly agree with the discussion of FID scores.

\mypara{Comparison with baselines.} With very low privacy ($\varepsilon=10^6$), we see that DP-GAN-MI outperforms all other methods at $5$ out of the $6$ datasets, which shows that in the absence of privacy, GAN has the strongest ability to learn an arbitrary distribution. The FID scores of DP-DRE are close to DP-GAN-MI on all datasets; this suggests that the bias of DP-DRE is almost as small as that of a strong generative method such as a GAN. DP-MGE, in contrast, suffers from a larger bias, as is to be expected. 

%They are at most 4.7 higher than the scores of DP-GAN-MI.
%This argues that ImageNet is a promising public dataset for various private datasets, and more importantly, with a suitable public dataset, the bias of DP-DRE could be as small as a strong generative method such as GAN.
%However, DP-MGE suffers much larger bias than DP-GAN-MI on all datasets except the Car dataset. 
%Such large bias can come from the distance between the target distribution in the latent space and any gaussian distribution.

However, at higher privacy levels ($\varepsilon\leq 10$), our methods DP-MGE and DP-DRE fare better than all three baselines. DP-MEPF already has a large bias at $\varepsilon=10^6$ for all datasets except Cifar10. This might be because it is difficult to adapt to high resolution images. DP-GAN-FT and DP-GAN-MI also performs poorly with DP noise. The training process of GANs is known to be quite brittle, and so this might be because DP makes the training even harder. In contrast, DP-MGE and DP-DRE have more stable training processes, and hence they do better. 

%This shows the difficulty of DP-MEPF to be adapted to the high-resolution image dataset, while our methods built on strong pretrained IC-GAN naturally fit to the high-resolution image generation.
%Two methods with GAN, DP-GAN-FT and DP-GAN-MI are suddenly crashed when noises from DP are injected into the training.
%Indeed, it is known that the training process of GAN is very brittle and DP makes its training even harder, %\cite{xie2018differentially, jordon2018pate, long2021g, chen2020gs}
%while DP-MGE and DP-DRE have more stable training processes and smaller parameter spaces.

\mypara{Comparison between DP-MGE and DP-DRE.} Due to the simplicity of the multivariate gaussian distribution, we expect DP-MGE to have a larger bias than DP-DRE, but be more robust to noise due to DP. Indeed this is what we observe. On the large datasets (Cifar10 and Objects-Grass), DP-DRE is considerably better than DP-MGE while the methods are comparable in the smaller datasets. We suspect that DP-DRE performs well for low $\varepsilon$ because we use a simple MLP with a small hidden layer size. 

%the performance drops a little even when $\varepsilon=0.1$.
%On the remaining smaller datasets, the performance keeps mostly the same between $\varepsilon=10^6$ and $\varepsilon=1$.
%Thus, DP-MGE sometimes (e.g. on the Bird dataset) outperforms DP-DRE when $\varepsilon$ is small .

%DP-DRE has decent performance among all baselines when $\varepsilon=10^6$. 
%Because the model of DP-DRE in this experiment is only an MLP with relatively small hidden sizes, DP-DRE also has good robustness to the smaller $\varepsilon$.
%It performs the best in most settings of datasets and $\varepsilon$. 

\mypara{Image quality.} Figure~\ref{fig:examples} shows the randomly generated examples for each algorithm with $\varepsilon=10$. More examples with different $\varepsilon$ are in the Appendix. We see that DP-DRE and DP-MGE generate the most in-distribution images with high quality for all datasets except Object-Autumn. Other methods either generate many irrelevant out-of-distribution images (DP-GAN-FT, DP-GAN-MI) or have many artifacts (DP-MEPF). These artifacts may be due to the fact that DP-MEPF does not use a pretrained public encoder. By observing that on Object-Autumn even non-private IC-GAN doesn't generate perfect autumn-like images, we suspect that the anomalous performance in Object-Autumn is because the public feature extractor $h$ does not properly capture the features of \textit{autumn}.

\mypara{Sanity check for DP-DRE.} To see to what extent DP-DRE generates in-distribution images, we record the weights assigned by DP-DRE to images in the ImageNet validation set. For the Bird dataset, we sum up the weights for images belonging to the superclass \textit{bird}\footnote{The definition of superclass follows the ImageNet hierarchy at \url{https://observablehq.com/@mbostock/imagenet-hierarchy}}.
Similarly for the Car dataset, we sum up the weights belonging to the superclass \textit{wheeled vehicle} together with classes \{\textit{minibus}, \textit{school bus}, \textit{trolleybus}, \textit{car wheel}\}.
Table~\ref{tab:weight} shows the weights for these two datasets.
When the $\varepsilon\in\{10^6, 10\}$ for the Bird dataset and the $\varepsilon\in\{10^6, 10, 3, 1\}$ for the Car dataset, we see the weights are all above $95\%$. This indicates that at least $95\%$ of the images generated are close to that of Birds or Cars. 

\begin{table}[t]
	\centering
	\begin{tabular}{c|ccccc}
	\toprule
		& $\varepsilon=10^6$ & $\varepsilon=10$ & $\varepsilon=3$ & $\varepsilon=1$ & $\varepsilon=0.1$\\
	\midrule
	Bird &	0.98 & 0.96 & 0.85 & 0.40 & 0.06\\
	Car & 0.98 & 0.97 & 0.98 & 0.96 & 0.05\\
	\bottomrule
	\end{tabular}
	\caption{The weight assigned to same semantic superclass.}
	\label{tab:weight}
\end{table}

